Analytic reconstruction with massive particles: one-loop amplitudes for $0 \to \bar{q}qt\bar{t}H$

We present an analytic reconstruction of one-loop amplitudes for the process $0 \to \bar{q}qt\bar{t}H$. Our calculation is a novel use of analytic reconstruction, retaining explicit covariance in the massive spin states through the massive spinor-helicity formalism. The analytic reconstruction relies on embedding the massive five-point kinematics in a fully massless eight-point phase space while still building a minimal ansatz directly in the five-point phase space. In order to obtain compact analytic expressions it is necessary to identify suitable partial fraction decompositions and extract common numerator factors, which we achieve through careful inspection of limits in which pairs of denominators vanish. We find that the resulting amplitudes are more numerically efficient than ones computed using automatic methods but that the gains are not as significant as in the massless case, at least at present. The method opens the door to applications at two-loop order, where numerical efficiency and improvements in the reconstruction methodology are more crucial, especially with regards to the number of free parameters in the ansatz.

==> makefile <==
FC = gfortran
HERE   = $(PWD)

FFLAGS = -ffixed-line-length-none
DIRS	= $(HERE)

# -----------------------------------------------------------------------------

# Specify the object files. 

qbqttbHFILES= \
precision.o \
slashify.o \
spinorzero_generic.o \
spinorfunctions.o \
zprod_generic.o \
ubarKS.o \
vKS.o \
dotc.o \
QuarkString.o \
loqbqttH.o \
ctqbqttH.o \
d3x4x12xm0mm_sym.o \
d3x4x12xm0mm.o \
d3x12x4xm00m_unsym.o \
d3x12x4xm00m.o \
d3x1x24xm00m_guts.o \
d3x1x24xm00m.o \
d3x2x14xm00m.o \
d4x2x1xm000_guts.o \
d4x2x1xm000.o \
d4x1x2xm000.o \
c1x23x00m_guts.o \
c1x23x00m.o \
c2x13x00m.o \
c12x3xmm0.o \
c12x3x00m_sym.o \
c12x3x00m_unsym.o \
c12x3x00m.o \
c12x34xmmm_unsym.o \
c12x34xmmm_sym.o \
c12x34xmmm.o \
c124x3xm0m_guts.o \
c124x3xm0m.o \
c13x24xm0m_guts.o \
c13x24xm0m_sym.o \
c13x24xm0m.o \
c14x23xm0m.o \
triangle_irsub.o \
b12x00.o \
b12x00_halfsym.o \
b12x00_fullsym_nobox.o \
b12x00_fullsym_box.o \
b12xmm_unsym.o \
b12xmm_unsym_noboxgram.o \
b12xmm_unsym_boxgram.o \
b12xmm.o \
b123xm0_asym.o \
b123xm0_sym.o \
b123xm0.o \
b13xm0_guts.o \
b13xm0.o \
b34xmm.o \
b1234xmm.o \
b23xm0.o \
ttHrat.o \
bub3xm0rel.o \
zabfill.o \
newcoeffs_irsub.o \
checkcoeffs.o \
qbqttbH.o


.f.o: 	
		$(FC) $(FFLAGS) -c $< 

# -----------------------------------------------------------------------------

qbqttbH:  \
	$(qbqttbHFILES) 
	$(FC) $(FFLAGS)  -o $@ \
            $(qbqttbHFILES) 


# -----------------------------------------------------------------------------

clean: 
	- rm -f *.o *.mod *.s *.prj *~ core qbqttbH

# -----------------------------------------------------------------------------

# DO NOT DELETE
FTNCHEKPATH = /home/ellis/bin/
FORCHKPATH = /home/ellis/bin/

# Specify the dependencies of the .o files and the rules to make them.

FOROPTS = -include=$(INCPATH) -nonovice -nopretty -quiet

.SUFFIXES:  .prj

# improved so that .prj files are moved out of src directory and
# into base, only for .f files that don't already exist there
.f.prj:  
		$(FTNCHEKPATH)/ftnchek -project -noextern\
            $(FOROPTS) $< ; \
            if ! [ -e $(HERE)/$(notdir $<) ] ; then \
            mv $(basename $<).prj $(HERE) ; fi

PRJS =     $(TOTAL: .o=.prj) 

check:       $(PRJS) 
		$(FTNCHEKPATH)/ftnchek -Incdir $(INCPATH) $(FOROPTS) $(PRJS)



PRJSF =      $(TOTAL: .o=.f) 

checkf:       
		$(FORCHKPATH)/forchk  $(PRJSF)

# -----------------------------------------------------------------------------


QuarkString.o: weyl.f GR.f GL.f 
b1234xmm.o: b1234xmm.f mxpart.f b1234xmm_inc.f 
b123xm0_asym.o: mxpart.f b123xm0_asym_inc.f b123xm0_asym.f 
b123xm0.o: b123xm0.f 
b123xm0_sym.o: b123xm0_sym.f b123xm0_sym_inc.f mxpart.f 
b12x00.o: mxpart.f b12x00.f b12x00_inc.f 
b12x00_fullsym.o: sym.f 
b12xmm.o: b12xmm.f mxpart.f 
b12xmm_unsym.o: b12xmm_unsym.f b12xmm_unsym_inc.f 
b13xm0.o: b13xm0.f mxpart.f 
b13xm0_guts.o: b13xm0_guts.f 
b23xm0.o: mxpart.f b23xm0.f 
b34xmm.o: mxpart.f b34xmm.f b34xmm_inc.f 
bub3xm0rel.o: nflav.f 
c124x3xm0m.o: mxpart.f c124x3xm0m.f 
c124x3xm0m_guts.o: mxpart.f c124x3xm0m_sym_inc.f c124x3xm0m_asym_inc.f c124x3xm0m_guts.f 
c12x34xmmm.o: c12x34xmmm.f mxpart.f 
c12x34xmmm_sym.o: c12x34xmmm_sym.f mxpart.f 
c12x34xmmm_unsym.o: c12x34xmmm_unsym.f c12x34xmmm_unsym_inc.f 
c12x3x00m.o: c12x3x00m_unsym.f c12x3x00m_sym.f c12x3x00m.f mxpart.f c12x3x00m_sym_inc.f c12x3x00m_unsym_inc.f 
c12x3xmm0.o: c12x3xmm0.f mxpart.f c12x3xmm0_inc.f 
c13x24xm0m.o: c13x24xm0m.f mxpart.f c13x24xm0m_guts.f c13x24xm0m_sym.f 
c14x23xm0m.o: c14x23xm0m.f 
c1x23x00m.o: c1x23x00m.f mxpart.f 
c1x23x00m_guts.o: mxpart.f c1x23x00m_guts.f 
c1x3x00m.o: c1x3x00m.f 
c1x3x00m_guts.o: c1x3x00m_guts.f 
c2x13x00m.o: mxpart.f c2x13x00m.f 
c2x3x00m.o: c2x3x00m.f 
checkcoeffs.o: types.f ttHlabels.f weyl.f zabstrings.f 
ctqbqttH.o: mxpart.f 
d3x12x4xm00m.o: mxpart.f d3x12x4xm00m.f d3x12x4xm00m_unsym.f 
d3x1x24xm00m_guts.o: mxpart.f d3x1x24xm00m_guts.f 
d3x2x14xm00m.o: mxpart.f d3x2x14xm00m.f 
d3x4x12xm0mm.o: mxpart.f d3x4x12xm0mm.f 
d3x4x12xm0mm_sym.o: mxpart.f d3x4x12xm0mm_sym_inc.f d3x4x12xm0mm_sym.f 
d4x1x2xm000.o: d4x1x2xm000.f mxpart.f 
d4x2x1xm000_guts.o: mxpart.f d4x2x1xm000_guts.f 
dotc.o: dotc_inc.f mcfmnotation.f 
loqbqttH.o: mxpart.f 
newcoeffs_irsub.o: types.f mxpart.f constants.f ttHlabels.f zabstrings.f 
pol_mless.o: mcfmnotation.f 
precision.o: consts.f 
qbqttbH.o: types.f mxpart.f mcfmnotation.f nflav.f ttHlabels.f weyl.f zabstrings.f kinpoint_ggttH.f 
slashify.o: slashify_inc.f mcfmnotation.f weyl.f swapxz.f 
spinorfunctions.o: ubar_inc.f vl_inc.f pol_mless_inc.f 
spinorzero.o: vspinorzero_inc.f ubarspinorzero_inc.f uspinorzero_inc.f 
triangle_irsub.o: mxpart.f 
triangle_irsub.o: triangle_irsub.f 
ttHrat.o: ttHrat.f mxpart.f ttHrat_inc.f 
ubarKS.o: ubarKS_inc.f 
vKS.o: vKS_inc.f mcfmnotation.f weyl.f 
vspinorzero.o: mcfmnotation.f weyl.f swapxz.f 
zabfill.o: mxpart.f 




